Simple data balancing achieves competitive worst-group-accuracy

We study the problem of learning classifiers that perform well across (known or unknown) groups of data. After observing that common worst-group-accuracy datasets suffer from substantial imbalances, we set out to compare state-of-the-art methods to simple balancing of classes and groups by either subsampling or reweighting data. Our results show that these data balancing baselines achieve state-of-the-art-accuracy, while being faster to train and requiring no additional hyper-parameters. In addition, we highlight that access to group information is most critical for model selection purposes, and not so much during training. All in all, our findings beg closer examination of benchmarks and methods for research in worst-group-accuracy optimization.

==> tables/hparams.tex <==
\begin{table}[]
      \begin{tabular}{@{}llll@{}}
            \toprule
            \textbf{Algorithm}                & \textbf{Dataset}     & \textbf{Hyperparameters}    & \textbf{Grid}             \\ \midrule
            \multirow{7}{*}{All}              & \multirow{4}{*}{All} & learning rate               & 1e-5, 1e-4, 1e-3          \\
                                              &                      & momentum                    & 0, 0.5, 0.9               \\
                                              &                      & weight decay                & 1e-4, 1e-3, 1e-2, 1e-1, 1 \\ \cmidrule(l){2-4}
                                              & Waterbirds           & \multirow{4}{*}{Batch Size} & 2, 4, 8, 16, 32, 64, 128  \\
                                              & CelebA               &                             & 2, 4, 8, 16, 32, 64, 128  \\
                                              & MultiNLI             &                             & 2, 4, 8, 16, 32           \\
                                              & CivilComments        &                             & 2, 4, 8, 16, 32           \\ \midrule
            \multirow{5}{*}{Just Train Twice} & All                  & up                          & 4, 5, 6, 20, 50, 100      \\ \cmidrule(l){2-4}
                                              & Waterbirds           & \multirow{4}{*}{T}          & 40, 50, 60                \\
                                              & CelebA               &                             & 1, 5, 10                  \\
                                              & MultiNLI             &                             & 1, 2                      \\
                                              & CivilComments        &                             & 1, 2                      \\ \bottomrule
      \end{tabular}
      \caption{Search space of hyper-parameters. All hyperparameters are chosen by sampling uniformly.}
      \label{tab:hparam_search_space}
\end{table}

==> tables/result_time_h.tex <==
\begin{table}
    \begin{center}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{lllccccc}
                \toprule
                \textbf{Method} & \textbf{\#HP} & \textbf{Groups} & \multicolumn{4}{c}{\textbf{Time per epoch (minutes)}} & \textbf{Average}                                    \\
                \cmidrule(lr){4-7}
                                &               &                 & CelebA                                                & Waterbirds       & MultiNLI & CivilComments &       \\
                \midrule
                ERM             & 4             & No              & 15.28                                                 & 93.13            & 47.75    & 0.99          & 39.29 \\
                JTT             & 6             & No              & 25.97                                                 & 122.32           & 148.76   & 1.53          & 74.64 \\
                RWY             & 4             & No              & 15.41                                                 & 92.34            & 49.68    & 1.10          & 39.63 \\
                SUBY            & 4             & No              & 6.09                                                  & 23.96            & 47.87    & 0.68          & 19.65 \\
                \midrule
                RWG             & 4             & Yes             & 15.98                                                 & 52.46            & 63.19    & 1.04          & 33.17 \\
                SUBG            & 4             & Yes             & 1.65                                                  & 11.21            & 9.20     & 0.43          & 5.63  \\
                gDRO            & 5             & Yes             & 14.40                                                 & 92.85            & 49.44    & 1.00          & 39.42 \\
                \bottomrule
            \end{tabular}
        }
    \end{center}
    \caption{Median time per epoch for each method/dataset combination.
        The median is taken over all runs in the sweep.
        \#HP is the number of hyper-parameters tuned.
        Simple baselines, while performing similarly, take drastically less time to train.}
    \label{table:time}
\end{table}



==> tables/result_worst_acc_low_reg.tex <==
\begin{table}
    \begin{center}
        \setlength{\aboverulesep}{0pt}
        \setlength{\belowrulesep}{0pt}
        \setlength{\extrarowheight}{.75ex}
        \resizebox{\textwidth}{!}{

            \begin{tabular}{lllccccc}
                \toprule
                \textbf{Method} & \textbf{\#HP} & \textbf{Groups} & \multicolumn{4}{c}{\textbf{Worst Acc}} & \textbf{Average}                                       \\
                \cmidrule(lr){4-7}
                                &               &                 & CelebA                                 & Waterbirds       & MultiNLI     & CivilComments &      \\
                \midrule
                ERM             & 4             & No              & 47.8$\pm$5.2                           & 81.7$\pm$2.5     & 67.1$\pm$0.9 & 59.9$\pm$0.9  & 64.1 \\
                JTT             & 6             & No              & 57.7$\pm$7.3                           & 84.8$\pm$1.8     & 58.9$\pm$0.6 & 55.3$\pm$2.4  & 64.2 \\
                RWY             & 4             & No              & 66.4$\pm$1.9                           & 76.5$\pm$3.6     & 66.5$\pm$1.2 & 69.5$\pm$0.8  & 69.7 \\
                SUBY            & 4             & No              & 67.7$\pm$3.9                           & 75.7$\pm$5.9     & 54.9$\pm$0.6 & 45.9$\pm$1.4  & 61.1 \\
                \midrule
                RWG             & 4             & Yes             & 51.2$\pm$4.5                           & 80.2$\pm$3.6     & 64.9$\pm$0.8 & 69.4$\pm$0.5  & 66.4 \\
                SUBG            & 4             & Yes             & 86.1$\pm$2.9                           & 88.1$\pm$0.8     & 68.4$\pm$0.6 & 66.6$\pm$2.1  & 77.3 \\
                gDRO            & 5             & Yes             & 69.6$\pm$3.2                           & 77.6$\pm$2.6     & 76.3$\pm$1.3 & 57.4$\pm$10.4 & 70.2 \\

                \bottomrule                                                                                                                                         \\
            \end{tabular}
        }
    \end{center}
    \caption{Test worst-group-accuracy for all methods and datasets with weight decay = $1e-4$ and last epoch chosen.}
    \label{table:accuracy_mean_selec}
\end{table}


==> tables/result_worst_acc_mean_selec.tex <==
\begin{table}
    \begin{center}
        \setlength{\aboverulesep}{0pt}
        \setlength{\belowrulesep}{0pt}
        \setlength{\extrarowheight}{.75ex}
        \resizebox{\textwidth}{!}{
 
            \begin{tabular}{lllccccc}
                \toprule
                \textbf{Method} & \textbf{\#HP} & \textbf{Groups} & \multicolumn{4}{c}{\textbf{Worst Acc}} & \textbf{Average}                                       \\
                \cmidrule(lr){4-7}
                                &               &                 & CelebA                                 & Waterbirds       & MultiNLI     & CivilComments &      \\
                \midrule
                ERM             & 4             & No              & 37.4$\pm$4.2                           & 82.8$\pm$1.5     & 63.6$\pm$2.1 & 47.8$\pm$2.9  & 57.9 \\
                JTT             & 6             & No              & 39.7$\pm$5.2                           & 79.9$\pm$2.3     & 57.5$\pm$4.3 & 40.7$\pm$7.1  & 54.4 \\
                RWY             & 4             & No              & 46.9$\pm$7.1                           & 75.6$\pm$2.3     & 66.5$\pm$1.2 & 63.5$\pm$1.8  & 63.1 \\
                SUBY            & 4             & No              & 40.0$\pm$7.5                           & 78.9$\pm$4.2     & 61.9$\pm$2.9 & 0.0$\pm$0.0   & 45.2 \\
                \midrule
                RWG             & 4             & Yes             & 47.9$\pm$2.5                           & 79.3$\pm$1.9     & 63.6$\pm$0.3 & 53.9$\pm$3.5  & 61.2 \\
                SUBG            & 4             & Yes             & 60.2$\pm$5.0                           & 85.5$\pm$0.7     & 67.8$\pm$1.8 & 59.8$\pm$6.1  & 68.4 \\
                gDRO            & 5             & Yes             & 43.4$\pm$2.5                           & 81.9$\pm$1.9     & 76.3$\pm$1.3 & 60.9$\pm$8.3  & 65.6 \\
                \bottomrule                                                                                                                                         \\
            \end{tabular}
        }
    \end{center}
    \caption{Test worst-group-accuracy for all methods and datasets. \#HP is the number of hyper-parameters tuned.
        These are the results when selecting model based on their average validation accuracy instead of the worst validation accuracy.
        This underlines the importance of specifying the problem at hand (\cite{damour2020Underspecification}).
        Just by using a few group annotated validation samples one can have a much better performing model, even if it wasn't trained using group information.
    }
    \label{table:accuracy_mean_selec}
\end{table}

